A quantum Frucht's theorem and quantum automorphisms of quantum Cayley graphs

We establish a quantum version of Frucht's Theorem, proving that every finite quantum group is the quantum automorphism group of an undirected finite quantum graph. The construction is based on first considering several quantum Cayley graphs of the quantum group in question, and then providing a method to systematically combine them into a single quantum graph with the right symmetry properties. We also show that the dual $\widehat \Gamma$ of any non-abelian finite group $\Gamma$ is ``quantum rigid''. That is, $\widehat \Gamma$ always admits a quantum Cayley graph whose quantum automorphism group is exactly $\widehat \Gamma$.

==> strdiag.tex <==
%Some macros for typesetting string diagrams
%Daniel Gromada, 2024

\usetikzlibrary{decorations.markings}
\usetikzlibrary{shapes.geometric} 
\usetikzlibrary{shapes.symbols} 
\def\Dcup{\Diagram{\draw (1,1) .. controls +(down:0.5) and +(down:0.5) .. (2,1);}}
\def\Dcap{\Diagram{\draw (1,0) .. controls +(up:0.5) and +(up:0.5) .. (2,0);}}
\def\Did{\Diagram{\draw (1,0) -- (1,1);}}
\def\Dcross{\Diagram{\draw (0,0) -- (1,1);\draw (1,0) -- (0,1);}}

\def\Rcup{\Diagram{\draw[mid arrow] (1,1) .. controls +(down:0.5) and +(down:0.5) .. (2,1);}}
\def\Lcup{\Diagram{\draw[mid arrow] (2,1) .. controls +(down:0.5) and +(down:0.5) .. (1,1);}}
\def\Rcap{\Diagram{\draw[mid arrow] (1,0) .. controls +(up:0.5) and +(up:0.5) .. (2,0);}}
\def\Lcap{\Diagram{\draw[mid arrow] (2,0) .. controls +(up:0.5) and +(up:0.5) .. (1,0);}}
\def\Fid{\Diagram{\draw[mid arrow] (1,0) -- (1,1);}}
\def\Bid{\Diagram{\draw[mid arrow] (1,1) -- (1,0);}}

\def\textchoice#1#2#3#4#5{\ifmmode\mathchoice{#1}{#2}{#3}{#4}\else #5\fi}

\def\Diagram#1{%
\thinspace\textchoice
{\DiagramA{0.25em}{1em}{1em}{#1}}
{\DiagramA{0.25em}{0.7em}{1em}{#1}}
{\DiagramA{0.175em}{0.55em}{0.7em}{#1}}
{\DiagramA{0.125em}{0.4em}{0.5em}{#1}}
{\DiagramA{0.25em}{0.7em}{1em}{#1}}%
\thinspace%
}

\def\DiagramA#1#2#3#4{%
%\expandafter\tikzpicture\Gparam
\tikzpicture[
	%arrow styles
	mid arrow/.style={postaction={decorate,decoration={
        markings,
        mark=at position .5 with {\arrow{>}}
      }}},
	late arrow/.style={postaction={decorate,decoration={
        markings,
        mark=at position .8 with {\arrow{>}}
      }}},
	%point styles
	circ/.style={circle,draw,fill=white,inner sep=1pt},
	bcirc/.style={circle,draw,fill=black,inner sep=1pt},
	map/.style={draw,fill=white,trapezium,trapezium left angle=90,trapezium right angle=120,inner sep=1pt},
	mapC/.style={draw,fill=white,trapezium,trapezium left angle=120,trapezium right angle=90,inner sep=1pt},
	mapT/.style={draw,fill=white,trapezium,trapezium left angle=60,trapezium right angle=90,inner sep=1pt},
	mapA/.style={draw,fill=white,trapezium,trapezium left angle=90,trapezium right angle=60,inner sep=1pt},
	selfC/.style={draw,fill=white,trapezium,trapezium left angle=120,trapezium right angle=120,inner sep=1pt},
	selfCR/.style={draw,fill=white,trapezium,trapezium left angle=60,trapezium right angle=60,inner sep=1pt},
	selfT/.style={draw,fill=white,trapezium,trapezium left angle=60,trapezium right angle=120,inner sep=1pt},
	selfTR/.style={draw,fill=white,trapezium,trapezium left angle=120,trapezium right angle=60,inner sep=1pt},
	selfA/.style={draw,fill=white,signal,signal to=east,inner sep=1pt},
	selfAR/.style={draw,fill=white,signal,signal to=west,inner sep=1pt},
	square/.style={draw,fill=white,rectangle,inner sep=1pt},
	vec/.style={draw,fill=white,isosceles triangle, shape border rotate=-90,isosceles triangle apex angle=60,inner sep=1pt},
	covec/.style={draw,fill=white,isosceles triangle, shape border rotate=90,isosceles triangle apex angle=60,inner sep=1pt},
]
\pgfsetbaseline{#1}
\pgfsetxvec{\pgfpoint{#2}{0em}}
\pgfsetyvec{\pgfpoint{0em}{#3}}
\pgfsetlinewidth{\Dlinewidth em}
#4
\endtikzpicture
}

\def\Dlinewidth{0.05}

\def\DstringsB #1/#2(#3,#4){
\ifnum#1>0
\pgfmathparse{#3-(#1-1)/2}
\let\x=\pgfmathresult
\pgfmathparse{#3+(#1-1)/2}
\let\xx=\pgfmathresult
\foreach \a in {\x,...,\xx}
	\draw (\a,#4-\Dyshift) .. controls +(up:0.25) .. (#3,#4);
\fi
\ifnum#2>0
\pgfmathparse{#3-(#2-1)/2}
\let\x=\pgfmathresult
\pgfmathparse{#3+(#2-1)/2}
\let\xx=\pgfmathresult
\foreach \a in {\x,...,\xx}
	\draw (\a,#4+\Dyshift) .. controls +(down:0.25) .. (#3,#4);
\fi
}

\newcount\tmpcount
\def\Dcount#1{\ifx/#1/\else\advance\tmpcount by1\fihere\Dcount\fi}

\def\DstringsC [#1/#2](#3,#4){
\tmpcount=-1
\Dcount#1//
\pgfmathparse{#3-\the\tmpcount/2}
\let\x=\pgfmathresult
\scope[
	up arrow/.style={postaction={decorate,decoration={
        markings,
        mark=at position .3 with {\arrow{>}}
      }}},
	down arrow/.style={postaction={decorate,decoration={
        markings,
        mark=at position .3 with {\arrow{<}}
      }}},
]
\DstringsD{#3}{#4}#1//
\endscope
\tmpcount=-1
\Dcount#2//
\pgfmathparse{#3-\the\tmpcount/2}
\let\x=\pgfmathresult
\scope[
	down arrow/.style={postaction={decorate,decoration={
        markings,
        mark=at position .7 with {\arrow{>}}
      }}},
	up arrow/.style={postaction={decorate,decoration={
        markings,
        mark=at position .7 with {\arrow{<}}
      }}},
]
\DstringsE{#3}{#4}#2//
\endscope
}

\def\fihere#1\fi{\fi#1}
\def\DstringsD#1#2#3{\ifx/#3/\else
	\csname D#3\endcsname (\x,#2-\Dyshift) .. controls +(up:0.25) .. (#1,#2);
	\pgfmathparse{\x+1}
	\let\x=\pgfmathresult
	\fihere\DstringsD{#1}{#2}\fi
}
\def\DstringsE#1#2#3{\ifx/#3/\else
	\csname D#3\endcsname (\x,#2+\Dyshift) .. controls +(down:0.25) .. (#1,#2);
	\pgfmathparse{\x+1}
	\let\x=\pgfmathresult
	\fihere\DstringsE{#1}{#2}\fi
}

\def\Dstrings{
\futurelet\nextchar\DstringsA
}

\def\DstringsA{\ifx[\nextchar\let\next=\DstringsC\else\let\next=\DstringsB\fi\next}

\def\Dmor#1#2 (#3,#4){
\def\Dyshift{0.5}
\ifx;#2;\else\Dstrings#2(#3,#4)\fi
\node at (#3,#4) [#1] {};
}

\def\DMor#1#2 (#3,#4)#5{
\def\Dyshift{1}
\ifx;#2;\else\Dstrings#2(#3,#4)\fi
\node at (#3,#4) [#1] {#5};
}

\def\spider{\futurelet\nextchar\spiderA}
\def\spiderA{\ifx[\nextchar\def\next[##1]{\Diagram{\Dmor{bcirc}[##1] (1,0.5)}}\else\def\next##1{\Diagram{\Dmor{bcirc}##1 (1,0.5)}}\fi\next}
\def\wspider{\futurelet\nextchar\wspiderA}
\def\wspiderA{\ifx[\nextchar\def\next[##1]{\Diagram{\Dmor{circ}[##1] (1,0.5)}}\else\def\next##1{\Diagram{\Dmor{circ}##1 (1,0.5)}}\fi\next}

\def\Ddef#1#2{\expandafter\def\csname D#1\endcsname{#2}}
\Ddef>{\draw[<-]}
\Ddef<{\draw[>-]}
\Ddef-{\draw}
\Ddef={\draw[very thick]}
\expandafter\def\csname D0\endcsname#1;{}
\expandafter\def\csname D.\endcsname (#1,#2)#3;{\node at (#1,#2) {$\dots$};}

\endinput

